T2FPV: Dataset and Method for Correcting First-Person View Errors in Pedestrian Trajectory Prediction

Predicting pedestrian motion is essential for developing socially-aware robots that interact in a crowded environment. While the natural visual perspective for a social interaction setting is an egocentric view, the majority of existing work in trajectory prediction therein has been investigated purely in the top-down trajectory space. To support first-person view trajectory prediction research, we present T2FPV, a method for constructing high-fidelity first-person view (FPV) datasets given a real-world, top-down trajectory dataset; we showcase our approach on the ETH/UCY pedestrian dataset to generate the egocentric visual data of all interacting pedestrians, creating the T2FPV-ETH dataset. In this setting, FPV-specific errors arise due to imperfect detection and tracking, occlusions, and field-of-view (FOV) limitations of the camera. To address these errors, we propose CoFE, a module that further refines the imputation of missing data in an end-to-end manner with trajectory forecasting algorithms. Our method reduces the impact of such FPV errors on downstream prediction performance, decreasing displacement error by more than 10% on average. To facilitate research engagement, we release our T2FPV-ETH dataset and software tools.

==> sections/trajectory_prediction_method.tex <==
\section{TRAJECTORY PREDICTION METHODS}

% \soonmin{Do we need this section? We can better explain the baseline methods we used in Experiments section. In this section, we have to explain the proposed correction module.}

% \subsection{Baseline Approach Study}

% We implemented several representative approaches on the ETH/UCY trajectory prediction task as baselines to examine task performance. We selected these algorithms as they appear to stand out along several key techniques common in human trajectory prediction, such as variational prediction, social awareness, and goal conditioning. This approach led us to select VRNN~\cite{vrnn}, A-VRNN~\cite{acvrnn}, and SGNet~\cite{sgnet} as our initial algorithms to examine.

% Note that A-VRNN is an ablation of AC-VRNN, which adds in goal conditioning in a somewhat similar manner to SGNet, but ultimately performs worse in reported results; hence, we did not include it in our study. Additionally, while there are performers on the ETH/UCY benchmark leaderboard which report performing better than SGNet, as discussed in Section \ref{sec:rel_work}, they generally rely on additional input modalities beyond the scope of our task. Additional approaches would certainly be interesting to incorporate and study as well, but we leave this as future work extending beyond the scope of this study. \soonmin{Seems wordy?}

% \subsection{Our Approach}

% %After implementing and testing these baselines, we examined several potential means of further improving results and training stability. 
% To improve training stability, we employ
% %The first technique was incorporating 
% layer normalization (LN)~\cite{layernorm} after each hidden layer within the Multi-Layer Perceptron (MLP) blocks. This was motivated by works purporting its success in recurrent architectures, especially in recent Transformer-based approaches \cite{transformer}. Correction module architecture shown in Fig. \ref{fig:arch}.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/corr_arch.jpg}
\caption{(Placeholder, figures will be updated soon) Correction Module Architecture}\vspace{-0.3cm}%
    \label{fig:arch}
\end{figure}


% We also re-examined the methods of social awareness used, beyond GAT sub-networks~\cite{srlstm}. This technique was especially important when trying to improve SGNet~\cite{sgnet}, since their approach has no method of social awareness built in. In particular, besides graph-based social methods, other works have attempted pooling approaches \cite{slstm,sgan}. We thus created a version of social pooling that incorporates lessons learned from GAT and hidden state-refinement approaches~\cite{srlstm}: use a similarity adjacency matrix, based on closeness to other people in the scene at each timestep, to perform a weighted average pooling over others' hidden states to refine each agent's own hidden state. 

